Spherical Inducing Features for Orthogonally-Decoupled Gaussian Processes

Despite their many desirable properties, Gaussian processes (GPs) are often compared unfavorably to deep neural networks (NNs) for lacking the ability to learn representations. Recent efforts to bridge the gap between GPs and deep NNs have yielded a new class of inter-domain variational GPs in which the inducing variables correspond to hidden units of a feedforward NN. In this work, we examine some practical issues associated with this approach and propose an extension that leverages the orthogonal decomposition of GPs to mitigate these limitations. In particular, we introduce spherical inter-domain features to construct more flexible data-dependent basis functions for both the principal and orthogonal components of the GP approximation and show that incorporating NN activation features under this framework not only alleviates these shortcomings but is more scalable than alternative strategies. Experiments on multiple benchmark datasets demonstrate the effectiveness of our approach.

==> figures/uci_regression_additional/rmse_summary.tex <==
\begin{tabular}{lllll}
\toprule
                                       & inducing variable & \textsc{relu} features & \textsc{softplus} features & inducing points \\
                                       & kernel &                 Arccos &                     Arccos &          Arccos \\
dataset & \textsc{svgp} ($M$ inducing variables, $K$ orthogonal inducing variables) &                        &                            &                 \\
\midrule
\multirow{3}{*}{\textsc{boston} ($N=455, D=13$)} & $M=128, K=0$ &          $3.08\pm0.35$ &              $3.01\pm0.41$ &   $2.93\pm0.45$ \\
                                       & $M=128, K=128$ &          $2.48\pm0.24$ &              $2.48\pm0.24$ &   $2.85\pm0.42$ \\
                                       & $M=256, K=0$ &          $3.01\pm0.43$ &              $2.96\pm0.40$ &   $2.87\pm0.39$ \\
\cline{1-5}
\multirow{3}{*}{\textsc{naval} ($N=10740, D=14$)} & $M=128, K=0$ &          $0.01\pm0.00$ &              $0.00\pm0.00$ &   $0.00\pm0.00$ \\
                                       & $M=128, K=128$ &          $0.00\pm0.00$ &              $0.00\pm0.00$ &   $0.00\pm0.00$ \\
                                       & $M=256, K=0$ &          $0.00\pm0.00$ &              $0.00\pm0.00$ &   $0.00\pm0.00$ \\
\cline{1-5}
\multirow{3}{*}{\textsc{protein} ($N=41157, D=9$)} & $M=128, K=0$ &          $4.81\pm0.03$ &              $4.71\pm0.04$ &   $4.21\pm0.04$ \\
                                       & $M=128, K=128$ &          $4.21\pm0.05$ &              $4.20\pm0.05$ &   $4.05\pm0.04$ \\
                                       & $M=256, K=0$ &          $4.70\pm0.04$ &              $4.63\pm0.04$ &   $4.05\pm0.04$ \\
\cline{1-5}
\multirow{3}{*}{\textsc{wine (red)} ($N=1439, D=11$)} & $M=128, K=0$ &          $0.63\pm0.04$ &              $0.62\pm0.04$ &   $0.61\pm0.04$ \\
                                       & $M=128, K=128$ &          $0.62\pm0.04$ &              $0.61\pm0.04$ &   $0.61\pm0.04$ \\
                                       & $M=256, K=0$ &          $0.63\pm0.04$ &              $0.62\pm0.04$ &   $0.61\pm0.04$ \\
\cline{1-5}
\multirow{3}{*}{\textsc{wine (white)} ($N=4408, D=11$)} & $M=128, K=0$ &          $0.70\pm0.01$ &              $0.69\pm0.02$ &   $0.68\pm0.01$ \\
                                       & $M=128, K=128$ &          $0.67\pm0.01$ &              $0.67\pm0.01$ &   $0.67\pm0.01$ \\
                                       & $M=256, K=0$ &          $0.70\pm0.02$ &              $0.68\pm0.02$ &   $0.67\pm0.01$ \\
\bottomrule
\end{tabular}


==> figures/uci_regression_sqrexp/nlpd_summary.tex <==
\begin{tabular}{lllllllllll}
\toprule
                              & inducing variable & \multicolumn{3}{l}{\textsc{relu} features} & \multicolumn{3}{l}{\textsc{softplus} features} & \multicolumn{3}{l}{inducing points} \\
                              & kernel &                 Arccos & Mat\'{e}rn-$\nicefrac{5}{2}$ &     Squared Exp &                     Arccos & Mat\'{e}rn-$\nicefrac{5}{2}$ &     Squared Exp &          Arccos & Mat\'{e}rn-$\nicefrac{5}{2}$ &     Squared Exp \\
dataset & \textsc{svgp} ($M$ inducing variables, $K$ orthogonal inducing variables) &                        &                              &                 &                            &                              &                 &                 &                              &                 \\
\midrule
\multirow{3}{*}{\textsc{concrete} ($N=927, D=8$)} & $M=128, K=0$ &          $3.33\pm0.04$ &                $3.36\pm0.02$ &   $3.36\pm0.03$ &              $3.31\pm0.04$ &                $3.36\pm0.03$ &   $3.35\pm0.03$ &   $3.30\pm0.05$ &                $3.19\pm0.07$ &   $3.20\pm0.06$ \\
                              & $M=128, K=128$ &          $3.19\pm0.08$ &                $3.18\pm0.08$ &   $3.17\pm0.05$ &              $3.22\pm0.08$ &                $3.18\pm0.08$ &   $3.19\pm0.05$ &   $3.27\pm0.06$ &                $3.12\pm0.08$ &   $3.16\pm0.09$ \\
                              & $M=256, K=0$ &          $3.29\pm0.03$ &                $3.35\pm0.03$ &   $3.34\pm0.03$ &              $3.27\pm0.04$ &                $3.35\pm0.03$ &   $3.34\pm0.03$ &   $3.26\pm0.05$ &                $3.11\pm0.09$ &   $3.11\pm0.09$ \\
\cline{1-11}
\multirow{3}{*}{\textsc{energy} ($N=691, D=8$)} & $M=128, K=0$ &          $1.83\pm0.12$ &                $2.03\pm0.04$ &   $2.06\pm0.05$ &              $1.49\pm0.04$ &                $2.01\pm0.04$ &   $2.00\pm0.05$ &   $0.70\pm0.17$ &                $0.68\pm0.20$ &   $0.68\pm0.19$ \\
                              & $M=128, K=128$ &          $0.68\pm0.20$ &                $0.68\pm0.20$ &   $0.67\pm0.19$ &              $0.69\pm0.20$ &                $0.69\pm0.19$ &   $0.67\pm0.18$ &   $0.70\pm0.18$ &                $0.67\pm0.19$ &   $0.69\pm0.20$ \\
                              & $M=256, K=0$ &          $1.43\pm0.03$ &                $1.99\pm0.04$ &   $1.97\pm0.04$ &              $1.38\pm0.03$ &                $1.99\pm0.04$ &   $1.96\pm0.04$ &   $0.70\pm0.18$ &                $0.67\pm0.20$ &   $0.68\pm0.19$ \\
\cline{1-11}
\multirow{3}{*}{\textsc{kin8nm} ($N=7372, D=8$)} & $M=128, K=0$ &         $-0.69\pm0.02$ &               $-0.78\pm0.02$ &  $-0.61\pm0.02$ &             $-0.83\pm0.02$ &               $-0.82\pm0.02$ &  $-0.70\pm0.02$ &  $-0.85\pm0.02$ &               $-1.03\pm0.02$ &  $-1.07\pm0.02$ \\
                              & $M=128, K=128$ &         $-1.03\pm0.02$ &               $-1.03\pm0.02$ &  $-1.02\pm0.03$ &             $-1.03\pm0.02$ &               $-1.03\pm0.02$ &  $-1.02\pm0.03$ &  $-0.90\pm0.01$ &               $-1.10\pm0.02$ &  $-1.13\pm0.02$ \\
                              & $M=256, K=0$ &         $-0.89\pm0.02$ &               $-0.83\pm0.02$ &  $-0.76\pm0.02$ &             $-0.95\pm0.02$ &               $-0.84\pm0.02$ &  $-0.78\pm0.02$ &  $-0.90\pm0.01$ &               $-1.10\pm0.02$ &  $-1.13\pm0.02$ \\
\cline{1-11}
\multirow{3}{*}{\textsc{power} ($N=8611, D=4$)} & $M=128, K=0$ &          $2.85\pm0.04$ &                $2.86\pm0.03$ &   $2.86\pm0.04$ &              $2.85\pm0.04$ &                $2.86\pm0.03$ &   $2.86\pm0.04$ &   $2.79\pm0.04$ &                $2.78\pm0.05$ &   $2.80\pm0.05$ \\
                              & $M=128, K=128$ &          $2.80\pm0.05$ &                $2.80\pm0.05$ &   $2.82\pm0.04$ &              $2.79\pm0.05$ &                $2.80\pm0.05$ &   $2.82\pm0.04$ &   $2.77\pm0.04$ &                $2.73\pm0.05$ &   $2.78\pm0.05$ \\
                              & $M=256, K=0$ &          $2.85\pm0.04$ &                $2.86\pm0.03$ &   $2.86\pm0.04$ &              $2.85\pm0.04$ &                $2.86\pm0.03$ &   $2.86\pm0.04$ &   $2.77\pm0.05$ &                $2.73\pm0.05$ &   $2.76\pm0.05$ \\
\cline{1-11}
\multirow{3}{*}{\textsc{yacht} ($N=277, D=6$)} & $M=128, K=0$ &          $1.81\pm0.08$ &                $2.51\pm0.06$ &   $2.41\pm0.06$ &              $1.80\pm0.08$ &                $2.51\pm0.06$ &   $2.41\pm0.06$ &   $1.50\pm0.15$ &                $0.33\pm0.25$ &   $0.26\pm0.27$ \\
                              & $M=128, K=128$ &          $0.91\pm0.26$ &                $0.73\pm0.40$ &   $0.93\pm0.27$ &              $0.92\pm0.26$ &                $0.70\pm0.41$ &   $0.92\pm0.29$ &   $1.51\pm0.17$ &                $0.30\pm0.23$ &   $0.23\pm0.23$ \\
                              & $M=256, K=0$ &          $1.81\pm0.08$ &                $2.51\pm0.06$ &   $2.41\pm0.06$ &              $1.79\pm0.08$ &                $2.51\pm0.06$ &   $2.41\pm0.06$ &   $1.52\pm0.18$ &                $0.07\pm0.30$ &   $0.10\pm0.36$ \\
\bottomrule
\end{tabular}


==> figures/uci_regression_sqrexp/rmse_summary.tex <==
\begin{tabular}{lllllllllll}
\toprule
                              & inducing variable & \multicolumn{3}{l}{\textsc{relu} features} & \multicolumn{3}{l}{\textsc{softplus} features} & \multicolumn{3}{l}{inducing points} \\
                              & kernel &                 Arccos & Mat\'{e}rn-$\nicefrac{5}{2}$ &    Squared Exp &                     Arccos & Mat\'{e}rn-$\nicefrac{5}{2}$ &    Squared Exp &          Arccos & Mat\'{e}rn-$\nicefrac{5}{2}$ &    Squared Exp \\
dataset & \textsc{svgp} ($M$ inducing variables, $K$ orthogonal inducing variables) &                        &                              &                &                            &                              &                &                 &                              &                \\
\midrule
\multirow{3}{*}{\textsc{concrete} ($N=927, D=8$)} & $M=128, K=0$ &          $6.82\pm0.30$ &                $6.92\pm0.25$ &  $6.96\pm0.29$ &              $6.69\pm0.29$ &                $6.89\pm0.26$ &  $6.89\pm0.29$ &   $6.58\pm0.37$ &                $5.94\pm0.25$ &  $5.90\pm0.27$ \\
                              & $M=128, K=128$ &          $5.93\pm0.38$ &                $5.87\pm0.30$ &  $5.89\pm0.22$ &              $6.06\pm0.32$ &                $5.91\pm0.33$ &  $5.99\pm0.25$ &   $6.40\pm0.40$ &                $5.75\pm0.35$ &  $5.92\pm0.38$ \\
                              & $M=256, K=0$ &          $6.56\pm0.20$ &                $6.87\pm0.26$ &  $6.84\pm0.26$ &              $6.45\pm0.24$ &                $6.86\pm0.26$ &  $6.83\pm0.26$ &   $6.40\pm0.35$ &                $5.64\pm0.29$ &  $5.38\pm0.33$ \\
\cline{1-11}
\multirow{3}{*}{\textsc{energy} ($N=691, D=8$)} & $M=128, K=0$ &          $1.36\pm0.30$ &                $1.58\pm0.17$ &  $1.70\pm0.19$ &              $0.95\pm0.10$ &                $1.53\pm0.16$ &  $1.57\pm0.17$ &   $0.47\pm0.08$ &                $0.47\pm0.08$ &  $0.47\pm0.08$ \\
                              & $M=128, K=128$ &          $0.47\pm0.08$ &                $0.47\pm0.08$ &  $0.46\pm0.08$ &              $0.47\pm0.08$ &                $0.47\pm0.08$ &  $0.46\pm0.08$ &   $0.48\pm0.08$ &                $0.47\pm0.08$ &  $0.47\pm0.08$ \\
                              & $M=256, K=0$ &          $0.91\pm0.08$ &                $1.51\pm0.15$ &  $1.50\pm0.15$ &              $0.86\pm0.08$ &                $1.51\pm0.15$ &  $1.49\pm0.14$ &   $0.47\pm0.08$ &                $0.46\pm0.08$ &  $0.47\pm0.07$ \\
\cline{1-11}
\multirow{3}{*}{\textsc{kin8nm} ($N=7372, D=8$)} & $M=128, K=0$ &          $0.12\pm0.00$ &                $0.10\pm0.00$ &  $0.13\pm0.00$ &              $0.10\pm0.00$ &                $0.10\pm0.00$ &  $0.12\pm0.00$ &   $0.10\pm0.00$ &                $0.08\pm0.00$ &  $0.08\pm0.00$ \\
                              & $M=128, K=128$ &          $0.08\pm0.00$ &                $0.08\pm0.00$ &  $0.09\pm0.00$ &              $0.08\pm0.00$ &                $0.08\pm0.00$ &  $0.09\pm0.00$ &   $0.09\pm0.00$ &                $0.08\pm0.00$ &  $0.08\pm0.00$ \\
                              & $M=256, K=0$ &          $0.10\pm0.00$ &                $0.10\pm0.00$ &  $0.11\pm0.00$ &              $0.09\pm0.00$ &                $0.10\pm0.00$ &  $0.11\pm0.00$ &   $0.09\pm0.00$ &                $0.08\pm0.00$ &  $0.08\pm0.00$ \\
\cline{1-11}
\multirow{3}{*}{\textsc{power} ($N=8611, D=4$)} & $M=128, K=0$ &          $4.20\pm0.16$ &                $4.22\pm0.15$ &  $4.24\pm0.16$ &              $4.20\pm0.16$ &                $4.22\pm0.15$ &  $4.24\pm0.16$ &   $3.93\pm0.18$ &                $3.90\pm0.19$ &  $3.96\pm0.19$ \\
                              & $M=128, K=128$ &          $3.96\pm0.18$ &                $3.96\pm0.19$ &  $4.07\pm0.16$ &              $3.91\pm0.19$ &                $3.96\pm0.19$ &  $4.06\pm0.16$ &   $3.85\pm0.18$ &                $3.71\pm0.19$ &  $3.87\pm0.18$ \\
                              & $M=256, K=0$ &          $4.20\pm0.16$ &                $4.22\pm0.15$ &  $4.24\pm0.16$ &              $4.20\pm0.16$ &                $4.22\pm0.15$ &  $4.24\pm0.16$ &   $3.83\pm0.19$ &                $3.68\pm0.19$ &  $3.81\pm0.18$ \\
\cline{1-11}
\multirow{3}{*}{\textsc{yacht} ($N=277, D=6$)} & $M=128, K=0$ &          $1.17\pm0.36$ &                $2.43\pm0.54$ &  $2.26\pm0.47$ &              $1.16\pm0.36$ &                $2.43\pm0.54$ &  $2.26\pm0.47$ &   $1.06\pm0.24$ &                $0.34\pm0.19$ &  $0.36\pm0.15$ \\
                              & $M=128, K=128$ &          $0.59\pm0.23$ &                $0.51\pm0.25$ &  $0.62\pm0.22$ &              $0.60\pm0.23$ &                $0.49\pm0.29$ &  $0.61\pm0.22$ &   $1.06\pm0.23$ &                $0.34\pm0.19$ &  $0.37\pm0.15$ \\
                              & $M=256, K=0$ &          $1.16\pm0.35$ &                $2.43\pm0.54$ &  $2.26\pm0.47$ &              $1.13\pm0.36$ &                $2.43\pm0.54$ &  $2.26\pm0.47$ &   $1.07\pm0.23$ &                $0.28\pm0.14$ &  $0.29\pm0.11$ \\
\bottomrule
\end{tabular}

